Data-driven learning of non-autonomous systems

We present a numerical framework for recovering unknown non-autonomous dynamical systems with time-dependent inputs. To circumvent the difficulty presented by the non-autonomous nature of the system, our method transforms the solution state into piecewise integration of the system over a discrete set of time instances. The time-dependent inputs are then locally parameterized by using a proper model, for example, polynomial regression, in the pieces determined by the time instances. This transforms the original system into a piecewise parametric system that is locally time invariant. We then design a deep neural network structure to learn the local models. Once the network model is constructed, it can be iteratively used over time to conduct global system prediction. We provide theoretical analysis of our algorithm and present a number of numerical examples to demonstrate the effectiveness of the method.

==> Method_091019.tex <==
\section{Deep Neural Network Approximation} \label{sec:method}
The ODE \eqref{eq:ode} defines a map from the initial condition to the solution at $t=T$ as below.
\begin{equation*}
\x(T)=\PPhi_\f(\x_0, \aalpha(\cdot, \omega)|_{[0, T]}, T)
\end{equation*}
Suppose $\alpha(t, \omega)=\alpha_n$ for $t\in [t_n, t_{n+1}]$, then by the mean value theorem we have
\begin{align*}
\x_{n+1}&=\x_n+\int_{t_n}^{t_{n+1}} \f(\x(s), \aalpha(s, \omega))\, ds\\
&=\x_n+\f(\x(\tau), \aalpha(\tau, \omega)), \quad \tau\in [t_n, t_{n+1}]\\
&=\x_n+\f(\x(\tau), \aalpha_n)\\
&=\x_n+\f(\PPhi_\f(\x_n, \aalpha(\cdot, \omega)|_{[t_n, \tau]}, \Delta_n), \aalpha_n)\\
&=\x_n+\f(\PPhi_\f(\x_n, \aalpha_n, \Delta_n), \aalpha_n).
\end{align*} 

Then if we define the effective increment $\pphi_\f(\x_n, \aalpha_n, \Delta_n)=\f(\PPhi_\f(\x_n, \aalpha_n, \Delta_n), \aalpha_n)$, we have the following discrete flow map.
\begin{equation*}
\x_{n+1}=\x_n+\pphi_\f(\x_n, \aalpha_n, \Delta_n).
\end{equation*}

We want to use the neural network to approxiamte the effective increment $\pphi_\f(\x_n, \aalpha_n, \Delta_n)$.



\subsection{Single Parameters}

\subsection{Multiple Parameters}


\section{Uncertainty Quantification}

Epistemic uncertainty quantification...









==> Setup_091019.tex <==
\section{Problem Setup} \label{sec:setup}
We are interested in studying the following differential equation with stochastic parameters.

\begin{equation}
\label{eq:ode}
\frac{d}{dt}\x(t, \omega)=\f(\x, \aalpha(t, \omega)), \quad \x(0)=\x_0,
\end{equation}
where $\x \in \R^d$ are sate variables with coordinates 
$(x_1, x_2, \ldots, x_d)$ and $\aalpha(\omega)\in \R^l$ are time-dependent random parameters with coordinates $(\alpha_1(t, \omega), \alpha_2(t, \omega),\ldots, \alpha_l(t, \omega))$. 
We further assume that each state variable $x_i(t, \omega)\in [a_i, b_i]$ and each random parameter is contained in $[p_i, q_i]$ for any $t$ and $\omega$. For the random parameters, we assume they are piecewise constant in time and each parameter $\alpha_i(t, \omega)$ can be parameterized by a sequence of random vectors $(\Delta_i, a_i)$, where $\Delta_i\sim U(0, \Delta)$ and $a_i\sim U(0, a)$. If we define 
\begin{equation*}
	t_n=\sum_{i=1}^n \Delta_i
\end{equation*}
then the random parameter $\alpha_i(t,\omega)=a_n$ if $t_n\leq t< t_{n+1}$.
We are interested in quantifying the uncertainty in the solution $\x(T, \Delta_1, a_1, \Delta_2, a_2, \ldots, \Delta_N, a_N)$ for $T>0$.
